Model-based reinforcement corrosion prediction: Continuous calibration with Bayesian optimization and corrosion wire sensor data

Chloride-induced corrosion significantly contributes to the degradation of reinforced concrete structures, making accurate predictions of chloride migration and its effects on material durability critical. This paper explores two modeling approaches to estimate the effective diffusion coefficient for chloride transport. The first approach follows Gehlen's interpretable diffusion model, which is based on established physical principles and incorporates time and temperature dependencies in predicting chloride migration. The second approach is a neural network-based method, where the neural network approximates the effective diffusion coefficient. In a subsequent step, the calibrated models are used to predict the penetration depth of the critical chloride content, taking into account the uncertainty in the critical chloride content. The models are calibrated using experimental data measured by a wire sensor installed in a concrete test bridge. The calibration results are compared to effective diffusion coefficients derived from drilling dust samples. A comparison of both approaches reveals the advantages of the physics-based model in terms of transparency and interpretability, while the neural network model demonstrates flexibility and adaptability in data-driven predictions. This study emphasizes the importance of combining traditional and machine learning-based methods to improve the accuracy of chloride migration predictions in reinforced concrete.

==> contributions.tex <==
\section*{Relevant Publications (Wessels et al.) for the Second Phase} 

\begin{enumerate}[label=(\arabic*)]
    \item  Ulrich Römer, Stefan Hartmann, Jendrik-Alexander Tröger, David Anton, Henning Wessels, Moritz Flaschel, Laura De Lorenzis. "Reduced and All-at-Once Approaches for Model Calibration and Discovery in Computational Solid Mechanics“. Accepted by Applied Mechanics Review (2024).  \\
    \noindent \textbf{The paper reviews algorithms for parameter identification and discovery from full-field data.}
\end{enumerate}

\begin{enumerate}[label=(\arabic*)]
\setcounter{enumi}{1}
    \item  Gopal Agarwal, Jorge-Humberto Urrea-Quintero, Henning Wessels, Thomas Wick. "Parameter identification and uncertainty propagation of hydrogel coupled diffusion-deformation using POD-based reduced-order modeling“. Accepted by Computational Mechanics (2024). \\
    \noindent \textbf{The paper proposed proper orthogonal decomposition of a coupled chemo-mechanical problem for many-query engineering tasks. The application here is on additive manufacturing, but the formulation can also be adapted to species transport in corrosion.}
\end{enumerate}


\begin{enumerate}[label=(\arabic*)]
 \setcounter{enumi}{2} 
    \item Alexander Henkes, Leon Herrmann, Henning Wessels, and Stefan Kollmannsberger. “Generative Adversarial Networks Enable Outlier Detection and Property Monitoring for Additive Manufacturing of Complex Structures”. Accepted in Engineering Applications of Artificial Intelligence (2024). \\
    \noindent \textbf{The paper proposes a physics-agnostic anomaly detection approach based on generative adversarial neural networks. }
\end{enumerate}

\begin{enumerate}[label=(\arabic*)]
 \setcounter{enumi}{3}
    \item Alexander Henkes, Jason K Eshraghian, and Henning Wessels. “Spiking neural network for nonlinear regression”. In: Royal Society Open Science (2024).\\
    \noindent\textbf{The paper proposes spiking neural networks (SNN) for regression. SNN significantly reduce the energy demand, making them feasible for on-site analysis of monitoring data as part of embedded systems.}
\end{enumerate}

\begin{enumerate}[label=(\arabic*)]
 \setcounter{enumi}{4}
 \item Vahab B. Narouie, Henning Wessels, and Ulrich Römer. “Inferring Displacement Fields from Sparse Measurements Using the Statistical Finite Element Method”. In: Mechanical Systems and Signal Processing 200 (2023).  \\
 \noindent \textbf{The paper uses statFEM as a data assimilation strategy for digital twinning of mechanical problems. } 
\end{enumerate}


\begin{comment}
\begin{enumerate}[label=(\arabic*)]
 \setcounter{enumi}{5}
    \item Alexander Henkes and Henning Wessels. “Three-dimensional microstructure generation using generative adversarial neural networks in the context of continuum micromechanics”. In: Computer Methods in Applied Mechanics and Engineering 400 (2022). 29 citations on google scholar 
\end{enumerate}
\end{comment}

\noindent \textbf{The below contributions demonstrate expertise on physics-informed machine learning:}
\begin{enumerate}[label=(\arabic*)]
 \setcounter{enumi}{5}
    \item  Alexander Henkes, Henning Wessels, and Rolf Mahnken. “Physics informed neural networks for continuum micromechanics”. In: Computer Methods in Applied Mechanics and Engineering 393 (2022). 
    \item Henning Wessels, Christian Weißenfels, and Peter Wriggers. “The neural particle method - an updated Lagrangian physics informed neural network for computational fluid dynamics”. In: Computer Methods in Applied Mechanics and Engineering 368 (2020). 
\end{enumerate}
\textbf{The below preprint proposes a PINN formulation for efficient, repeated calibration from full-field data:}
\begin{enumerate}[label=(\arabic*)]
    \setcounter{enumi}{7}
    \item  David Anton, Jendrik-Alexander Tröger, Henning Wessels, Ulrich Römer, Alexander Henkes, Stefan Hartmann. "Deterministic and statistical calibration of constitutive models from full-field data with parametric physics-informed neural networks." In: arXiv preprint arXiv:2405.18311 (2024).
\end{enumerate}
